PTCMIL: Multiple Instance Learning via Prompt Token Clustering for Whole Slide Image Analysis

Multiple Instance Learning (MIL) has advanced WSI analysis but struggles with the complexity and heterogeneity of WSIs. Existing MIL methods face challenges in aggregating diverse patch information into robust WSI representations. While ViTs and clustering-based approaches show promise, they are computationally intensive and fail to capture task-specific and slide-specific variability. To address these limitations, we propose PTCMIL, a novel Prompt Token Clustering-based ViT for MIL aggregation. By introducing learnable prompt tokens into the ViT backbone, PTCMIL unifies clustering and prediction tasks in an end-to-end manner. It dynamically aligns clustering with downstream tasks, using projection-based clustering tailored to each WSI, reducing complexity while preserving patch heterogeneity. Through token merging and prototype-based pooling, PTCMIL efficiently captures task-relevant patterns. Extensive experiments on eight datasets demonstrate its superior performance in classification and survival analysis tasks, outperforming state-of-the-art methods. Systematic ablation studies confirm its robustness and strong interpretability. The code is released at https://github.com/ubc-tea/PTCMIL.

==> section/02-related_work.tex <==
\section{Related Works}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/4_method/SMILE_overview.pdf}
    \caption{Overview of SMILE. (a) The training pipeline of SMILE. (b) The Transformer encoder block structure. (c) The supervision of training the token labeler and their effects to the boundary of WSI instances. The token labeler can learn a distinct boundary with  hard negative token labeling\,(TL) term in the objective function.}
    \label{fig:SMILE_overview}
\end{figure*}

\subsection{MIL for WSI Analysis}
Multiple instance learning is an algorithm designed to predict diagnoses from giga-pixeled WSIs\,\cite{hu2023state}. 
Typically, MIL consists of an instance-level feature extractor and a bag-level aggregator, and numerous studies have made efforts to advance each stage\,\cite{gadermayr2022multiple,chen2022scaling,li2021dual,wang2022transformer}. 
Many studies have focused on improving the instance features that enter the bag-level aggregator\,\cite{zhao2020predicting,li2021dual,liu2023multiple}. 
Instead of obtaining patch features through a pre-trained CNN model, efforts have been made to attain more refined instance representations considering the characteristics of WSIs. 
Orthogonally, there have been studies aiming at enhancing the performance of MIL by improving the bag-level aggregator\,\cite{lu2021data,shao2021transmil,zhang2022dtfd,chen2022self}. 
The bag-level aggregator compiles information from all feature embeddings to output a prediction for the bag-level. 
Beyond the simple compilation of features from the instance bag, like Max-pooling and Mean-pooling, more advanced MIL aggregators have been developed with learnable parameters. 
Notably, the emergence of Vision Transformers has greatly influenced MIL\,\cite{shao2021transmil,chen2022self,chen2022scaling,li2023vision, ikromjanov2022whole,hossain2023region,shao2023hvtsurv}.
The use of class tokens in the ViT structure for image classification can operate effectively as a bag-level aggregator with little change \cite{shao2021transmil}. 
However, previous studies have fallen short in utilizing the rich information contained in the patch output tokens, aside from the class token.

% \label{sec:related_works}
% \subsection{MIL for WSI Analysis}
% % Non ViT-based MIL algorithm
% Bag-level MIL aims to use only bag-level labels to weakly-supervised learn from instances and aggregate instance features to predict bag-level labels. It can be divided into separate instance-level feature extractor and bag-level aggregator. Many previous works~\cite{lu2021data,li2021dual,shao2021transmil,zhang2022dtfd,chen2022self,chen2022self} have tried to improve the architecture of aggregators to better pool the instance features extracted with a model pretrained on ImageNet~\cite{deng2009imagenet}.~\cite{zhao2020predicting,li2021dual,chen2022scaling} also have attempted to get better instance representation with self-supervised learning, which are orthogonal to previous methods. 
% Recently, some works propose self-paced supervised contrastive learning~\cite{liu2023multiple}, iterative fine-tuning over feature extractor and aggregator~\cite{wang2023iteratively}, hard instance mining~\cite{tang2023multiple} and cluster constraints~\cite{wu2023improving} to involve instance-level guidance to the aggregator. Since ViT-based structure~\cite{shao2021transmil,chen2022self,chen2022scaling} shows superior performance on WSI analysis, we aim to explore the \bd{self-} guidance from the ViT structure. 
 
% \cite{zhang2023prompt} proposed a prompt learning method to partially fine-tune the ViT-based feature extractor to avoid heavy computation with millions of patches and overfitting. 
% \cite{tang2023multiple} proposed a hard instance mining strategy to boost the performance of aggregator \bd{want to say their objective is not related to improve patch features but we can learn better features in an implicit way}. This paper aims to get rid of the fine-tune of feature extractor, but to leverage dense supervision to learn better instance feature representations from an implicit way in the aggregator from a sub-optimal version of features extracted with ResNet50 pretrained on ImageNet.
% ViT-based MIL algorithm

% But previous ViT-based MIL didn't consider patch output toekns. 

\subsection{Token Labeling}
Token labeling, as introduced in~\cite{jiang2021all,zhao2023fully,xiao2023token}, offers an innovative approach to supplement image-level supervision for ViT architecture by adding dense supervision directly onto output patch tokens.
The original token labeling~\cite{jiang2021all} leveraged a pre-trained convolution neural network\,(CNN)~\cite{brock2021high,tan2019efficientnet} proficient in analogous classification tasks, to generate dense score maps.
These dense score maps serve as token labels, providing granular insights for each patch token.
Subsequently, STL~\cite{zhao2023fully} unified the model structure of token-labeler\,(teacher) and the down-stream model\,(student) with the same ViT architectures. 
This advancement transforms dense score maps into confidence scores, indicating the presence of a class within specific patches, thus aligning more closely with image labels and enhancing the quality of dense supervision.
The underlying principle of token labeling, akin to ReLabel~\cite{yun2021re}, is to utilize multiple labels for more effective learning supervision.
This training methodology, invoving both teacher and student models, shares similarities with knowledge distillation~\cite{touvron2021training,yuan2020revisiting} or self-distillation~\cite{yun2020regularizing,pham2022revisiting}.
However, the intrinsic difference is that token labeling includes the fine-grained labels and supervision to the pipeline, whereas ReLabel and distillation only consider the image-level supervision. 

==> section/03-preliminary.tex <==
\section{Preliminary}
\subsection{Multiple Instance Learning}
% Multiple instance learning (MIL) is a form of weakly supervised learning method where the training data consists of labeled bags, each containing multiple instances. 
% % In WSI classification (e.g., distinguishing abnormal vs normal slides), we formulate the MIL problem as follows.
% Each labeled WSI, with label $Y \! \in \! \{0~(\text{negative}), 1~(\text{positive})\}$, represents as a bag $B$ consisting of $N$ instances (\textit{e.g.}, patches) such that $B = \{(x_1, y_1), ..., (x_N, y_N)\}$.
% Each patch is denoted as $x_i$ for $i\in [N]$. Without fine-grained annotations on its patches, the labels of individual instances $y_i$ for $i\in [n]$ is unknown. However, the label of the bag is determined by the instance labels within it:

Multiple instance learning (MIL) is a form of weakly supervised learning method for WSI classification. 
Each labeled WSI, with label $Y \! \in \! \{0~(\text{negative}), 1~(\text{positive})\}$, represents as a bag $B$ consisting of $N$ instances (\textit{e.g.}, patches) such that $B = \{(x_1, y_1), ..., (x_N, y_N)\}$.
Each patch is denoted as $x_i$ for $i\in [N]$. 
Without fine-grained annotations on its patches, individual instance labels $y_i$ for $i\in [n]$ are unknown but, the bag's label is determined by the instance labels within it:
\begin{equation}
  Y =
  \begin{cases}
    1\text{,} & \text{if }~\exists~y_i \text{ such that } y_i = 1, i \in [N]\\
    0\text{,} & \text{otherwise}.
  \end{cases}
\end{equation}
Existing MIL methods in WSI classification \cite{gadermayr2022multiple} typically consist of two steps.
% : 1) feature extraction from individual patches and 2) the aggregation of these features to make predictions at the bag level. 

\noindent\textbf{Step 1: Feature extraction.}  In MIL, employing appropriate feature extraction techniques can emphasize the important features or structures within the data. 
A feature extractor function, $\phi(\cdot)$, transforms each raw instance $x_i$ into a lower-dimensional feature vector $v_i = \phi(x_i)$. 

\noindent\textbf{Step 2: Bag-level aggregation.} After feature extraction, the next step is to aggregate the features of the instances to infer the label of the bag.
The aggregation function $F(\cdot)$ takes the feature vectors of all instances within a bag as inputs and outputs bag label prediction $\hat{Y}=F(\{v_1, ..., v_N\})$.
% The aggregation function $F(\cdot)$ can take many forms, such as maximum, average, or learnable functions.
% This work focuses on improving step 2: optimizing a ViT-based learnable aggregation function for patch features generated from a fixed feature extractor.



\subsection{Token Labeling}

In ViT, both feature vectors and a class token are input to the encoder, and the bag label is predicted from the class token output by the final layer. Building on the ViT architecture, token labeling has been proposed as a training objective to leverage the substantial information in each image patch~\cite{jiang2021all,zhao2023fully}. 
This method involves assigning pseudo token labels to individual patch tokens.
% to enable knowledge distillation at the patch level. 
Token labeling enables ViT to harness a broader spectrum of image information~\cite{zhao2023fully}.

To implement dense supervision via token labeling, we utilize the patch tokens output from ViT.
For a given input image $X$, the ViT produces a set of the output tokens $\{\mathbf{T}_{cls}, \mathbf{T}_1, ..., \mathbf{T}_N\}$, where $\mathbf{T}_{cls}$ represents the class token and $\mathbf{T}_i$ denotes the patch token corresponding to the embedding vector of the $i$-th patch. 
Employing the output patch tokens and their corresponding pseudo token labels $\{\hat{y}_1,...,  \hat{y}_N\}$, the token labeling training objective can be defined as follows:
\begin{equation}
\mathcal{L}_{TL}=\frac{1}{N} \sum_{i=1}^N \mathcal{H}(\mathbf{T}_i, \hat{y}_i)
\end{equation}
The final loss function for training ViT model with the token labeling is:
\begin{equation}
\mathcal{L}_{Final}=\mathcal{H}(\mathbf{T}_{cls}, Y) + \beta \mathcal{L}_{TL}
\label{eq:token_labeling}
\end{equation}
where $\mathcal{H}$ is the softmax cross-entropy loss and  $\beta$ represents the hyperparameter that controls the weight of the token labeling objective.



==> tables/FLOPS.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
Method        & \#Param. & FLOPs & Acc \\
\midrule
ViT   & $1.58$M             & $279$M   & $92.83_{1.92}$                \\
%TransMIL   & $2.66$M             & $614$M   &   $93.58_{0.80}$             \\\hline
\textbf{PTCMIL ($C$= 5) }  & $1.59$M             & $735$M   &      $93.66_{1.40}$     \\
\textbf{PTCMIL ($C$= 7)}& $1.59$M    & $960$M  & $93.81_{1.02}$       \\
\bottomrule
\end{tabular}
\caption{Comparison of ViT  backbone and PTCMIL of accuracy, Parameters, and FLOPs on TGCA-NSCLC. The result is based on UNI feature. The input data size is set to (120, 1024). $C$ means the number of clusters.}
\label{tab:flops}
\end{table}



==> tables/ablation.tex <==
% \begin{table}[]
% \centering
% \caption{Ablation experiment ($\%$ for AUC and Acc) of clustering, merging (w/o means using prompt tokens, w/ means using merged prototype tokens), and pooling modules on TCGA-NSCLC (classification) and TCGA-CRC (survival) datasets. The result is based on CTransPath feature. The last row represents the performance of our method.}
% \label{tab:ablation}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccc|ccc|cc|c}
% \hline
% \multicolumn{2}{c|}{Clustering} & \multicolumn{2}{c|}{Merging} & \multicolumn{3}{c|}{Pooling} & \multicolumn{2}{c|}{TCGA-NSCLC} & TCGA-CRC \\ \hline
% \multirow{2}{*}{w/o} & \multicolumn{1}{c|}{\multirow{2}{*}{w/}} & \multirow{2}{*}{w/o} & \multirow{2}{*}{w/} & \multirow{2}{*}{pro} & \multirow{2}{*}{cls} & \multirow{2}{*}{pro + cls} & \multirow{2}{*}{AUC} & \multirow{2}{*}{Acc} & \multirow{2}{*}{c-index} \\ 
%  & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  \\ \hline
% $\checkmark$ & \multicolumn{1}{c|}{} & $-$  & $-$  & $-$ & $-$ & $-$ & $96.58_{0.45}$ & $90.87_{0.68}$ & $0.705_{0.07}$ \\ \hline
%  & \multicolumn{1}{c|}{$\checkmark$} & $\checkmark$ &  &  &  & $\checkmark$ & $96.77_{0.79}$ & $90.94_{1.87}$ & $0.685_{0.08}$ \\ \hline
%  & \multicolumn{1}{c|}{$\checkmark$} &  & $\checkmark$ & $\checkmark$ &  &  & $96.92_{0.72}$ & $91.77_{1.01}$ & $0.726_{0.07}$ \\
%  & \multicolumn{1}{c|}{$\checkmark$} &  & $\checkmark$ &  & $\checkmark$ &  & $96.44_{0.54}$ & $90.95_{0.87}$ & $0.706_{0.07}$ \\
%  & \multicolumn{1}{c|}{$\checkmark$} &  & $\checkmark$ &  & &  $\checkmark$ & \bm{$97.31_{0.67}$} & \bm{$92.17_{1.80}$} & \bm{$0.738_{0.09}$} \\ \hline
% \end{tabular}%
% }
% \end{table}


\begin{table}[]
\centering
\caption{Ablation of clustering, merging (w/o means using prompt tokens, w/ means using merged prototype tokens), and pooling modules on TCGA-NSCLC (classification) and TCGA-CRC (survival) datasets. The result is based on CTransPath feature. The last row represents the performance of our method.}
\label{tab:ablation}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{cccc|ccc|cc|c}
\hline
\multicolumn{2}{c|}{Clustering} & \multicolumn{2}{c|}{Merging} & \multicolumn{3}{c|}{Pooling} & \multicolumn{2}{c|}{TCGA-NSCLC} & TCGA-CRC \\ \hline
\multirow{2}{*}{w/o} & \multicolumn{1}{c|}{\multirow{2}{*}{w/}} & \multirow{2}{*}{w/o} & \multirow{2}{*}{w/} & \multirow{2}{*}{pro} & \multirow{2}{*}{cls} & \multirow{2}{*}{pro + cls} & \multirow{2}{*}{AUC} & \multirow{2}{*}{Acc} & \multirow{2}{*}{c-index} \\ 
 & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  \\ \hline
$\checkmark$ & \multicolumn{1}{c|}{} & $-$  & $-$  & $-$ & $-$ & $-$ & $96.58_{0.45}$ & $90.87_{0.68}$ & $0.705_{0.07}$ \\ \hline
 & \multicolumn{1}{c|}{$\checkmark$} & $\checkmark$ &  &  &  & $\checkmark$ & $96.77_{0.79}$ & $90.94_{1.87}$ & $0.685_{0.08}$ \\ \hline
 & \multicolumn{1}{c|}{$\checkmark$} &  & $\checkmark$ & $\checkmark$ &  &  & $96.92_{0.72}$ & $91.77_{1.01}$ & $0.726_{0.07}$ \\
 & \multicolumn{1}{c|}{$\checkmark$} &  & $\checkmark$ &  & $\checkmark$ &  & $96.44_{0.54}$ & $90.95_{0.87}$ & $0.706_{0.07}$ \\
\rowcolor{yellow} & \multicolumn{1}{c|}{$\checkmark$} &  & $\checkmark$ &  & &  $\checkmark$ & \bm{$97.31_{0.67}$} & \bm{$92.17_{1.80}$} & \bm{$0.738_{0.09}$} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/ablation_cls_token.tex <==
\begin{table}[!h]
\centering
\caption{Classification result (\%) of w/ and w/o the class token.}
\label{tab:ablation_cls}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|cc}
\toprule
&\multicolumn{2}{c|}{Camelyon16}&\multicolumn{2}{c}{TCGA-NSCLC}\\
&AUC&Acc&AUC&Acc\\
\midrule          
w/o cls token&$98.62\pm0.91$&$97.92\pm0.89$&$00.00\pm00.00$&$00.00\pm00.00$\\
w/ cls token&\bm{$99.60\pm 0.34$}&\bm{$ 98.60\pm 0.35$}&$\bm{98.42\pm 0.27}$&\bm{$93.66\pm 1.40$}\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/ablation_con_reg.tex <==
\begin{table}[!h]
\centering
\caption{Classification result (\%) of contrastive learning and regularization term for clustering.}
\label{tab:ablation_con_reg}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|cc}
\toprule
&\multicolumn{2}{c|}{Camelyon16}&\multicolumn{2}{c}{TCGA-NSCLC}\\
&AUC&Acc&AUC&Acc\\
\midrule          
Contrastive&$00.00\pm00.00$&$00.00\pm00.00$&$00.00\pm00.00$&$00.00\pm00.00$\\
Regularization&$00.00\pm00.00$&$00.00\pm00.00$&$00.00\pm00.00$&$00.00\pm00.00$\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/ablation_merging.tex <==
\begin{table}[!h]
\centering
\caption{Classification result (\%) of different prototype merging methods.}
\label{tab:ablation_merging}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|cc}
\toprule
&\multicolumn{2}{c|}{Camelyon16}&\multicolumn{2}{c}{TCGA-NSCLC}\\
&AUC&Acc&AUC&Acc\\
\midrule          
% Baseline (best) &$ $&$ $\\
Prompt tokens&$97.86\pm0.78$&$97.46\pm0.75$\\
Soft merging&$99.49\pm 0.49$&$97.50\pm 0.86$&$98.17\pm 0.57$&$92.83\pm 1.33$\\
Hard merging&\bm{$99.60\pm 0.34$}&\bm{$ 98.60\pm 0.35$}&$\bm{98.42\pm 0.27}$&$\bm{93.66\pm 1.40}$\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/adaptation.tex <==
\begin{table}[t!]
\centering
\caption{Adaptation experiment result (\%) of pre-training on TCGA-NSCLS, few-shot learning on Camelyon16 and pre-training on Camelyon16, few-shot on TCGA-NSCLS. The result is based on UNI feature. Bold highlights the best performance.}
\label{tab:adaptation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|cc}
\toprule
Pretrained on&\multicolumn{2}{c|}{TCGA-NSCLC}&\multicolumn{2}{c}{Camelyon16}\\
Fewshot on&\multicolumn{2}{c|}{Camelyon16}&\multicolumn{2}{c}{TCGA-NSCLC}\\\hline
&AUC&Acc&AUC&Acc\\
\midrule                    
% ABMIL&$50.84_{15.69}$&$47.34_{10.83}$&$running$\\
DSMIL \cite{li2021dual}&$65.57_{8.81}$&$62.97_{6.76}$&$83.88_{6.74}$&$75.47_{6.15}$\\
CLAM \cite{lu2021data}&$62.04_{10.63}$&$61.41_{4.12}$&$84.72_{5.36}$&$76.08_{5.15}$\\
% ViT&$58.32_{13.25}$&$52.97_{8.26}$&$66.53_{10.51}$&$60.83_{8.13}$\\
TransMIL \cite{shao2021transmil} 
&$57.28_{6.14}$&$53.44_{5.78}$&$66.00_{10.59}$&$61.36_{9.54}$\\
% DTFD-MIL&&&\\
ILRA \cite{xiang2023exploring}&$50.15_{12.59}$&$53.91_{7.35}$&$53.73_{10.79}$&$53.46_{6.96}$\\
MambaMIL \cite{yang2024mambamil}&$65.45_{10.14}$&$65.31_{7.17}$&$83.93_{5.71}$ & $75.62_{4.45}$\\
PTCMIL (ours)&\bm{$69.49_{10.27}$}&\bm{$67.03_{10.53}$}&\bm{$85.73_{3.42}$}&\bm{$77.36_{3.89}$}\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/comparison_w_vit.tex <==
\begin{table}[t!]
\centering
\caption{Comparison of PTCMIL and a two-layer ViT with hidden feature dimension 384 (cls token for prediction) on classification tasks.}
\label{tab:comparison_w_vit}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
 & \multicolumn{2}{c|}{Camelyon16} & \multicolumn{2}{c}{TCGA-NSCLC} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Model & AUC & Accuracy & AUC & Accuracy \\ 
\midrule
ViT ($\text{n}=2$,$\text{dim}=384$)&$99.42\pm0.52$&$96.75\pm1.11$&$98.08\pm0.31$&$92.83\pm1.92$  \\
PTCMIL&\bm{$99.60\pm0.34$}&\bm{$98.60\pm0.35$}&\bm{$98.42\pm0.27$}& \bm{$93.66\pm1.40$} \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/complexity.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lc}
\toprule
Method         & Complexity ($\sim$)  \\
\midrule
DPC-KNN \cite{zeng2022not} & $O(N^2)$      \\
K-Medoids \cite{marin2023token}&  $O(N^2)$      \\
ATC \cite{haurum2025agglomerative}&  $O(N^2)$      \\
\textbf{PTCMIL (Ours)}& \textbf{ $O(N)$ }     \\
\bottomrule
\end{tabular}
\caption{Comparison of complexity with other token clustering or token merging methods in ViT.}
\label{tab:complexity}
\end{table}



==> tables/survival.tex <==
\begin{table}[t]
\centering
\caption{Survival analysis result (c-index) of PTCMIL on TCGA-LUAD, TCGA-BLCA, TCGA-BRCA, TCGA-CRC. Bold highlights the best performance.}
\label{tab:survival}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\toprule
Method &LUAD&BLCA&BRCA&CRC\\
\midrule
% ABMIL \cite{ilse2018attention}&$0.571_{0.09}$&$0.587_{0.03}$&$0.651_{0.06}$&$0.547_{0.14}$\\
DSMIL \cite{li2021dual}&$0.659_{0.07}$&$0.586_{0.06}$&$0.720_{0.06}$&$0.696_{0.11}$\\
CLAM \cite{lu2021data}&$0.625_{0.12}$&$0.603_{0.06}$&$0.698_{0.03}$&$0.678_{0.09}$\\
% ViT&\underline{$0.673_{0.12}$}&$0.608_{0.04}$&$0.686_{0.06}$&$0.681_{0.07}$&\underline{$0.705_{0.07}$}\\
DTFD-MIL \cite{zhang2022dtfd}&&&&\\
TransMIL \cite{shao2021transmil}&$0.660_{0.12}$&{$0.616_{0.08}$}&$0.708_{0.05}$&$0.686_{0.06}$\\
% DTFD-MIL \cite{zhang2022dtfd}&\\
ILRA \cite{xiang2023exploring}&$\bm{0.688_{0.06}}$&$0.603_{0.04}$&$0.726_{0.08}$&${0.704_{0.09}}$\\
PANTHER \cite{Song_2024_CVPR}&$0.632_{0.07}$&$0.612_{0.07}$&{$0.729_{0.08}$}&$0.632_{0.14}$\\
MambaMIL \cite{yang2024mambamil}&$0.670_{0.08}$&$0.606_{0.04}$&$0.668_{0.05}$&$0.680_{0.06}$\\
DGR-MIL \cite{zhu2024dgr}&&&&\\
PTCMIL (ours)&\bm{$0.688_{0.09}$}&\bm{$0.630_{0.05}$}&\bm{$0.745_{0.04}$}&\bm{$0.738_{0.09}$}\\
\bottomrule
\end{tabular}}
\end{table}

